Image Masking for Robust Self-Supervised Monocular Depth Estimation

Self-supervised monocular depth estimation is a salient task for 3D scene understanding. Learned jointly with monocular ego-motion estimation, several methods have been proposed to predict accurate pixel-wise depth without using labeled data. Nevertheless, these methods focus on improving performance under ideal conditions without natural or digital corruptions. The general absence of occlusions is assumed even for object-specific depth estimation. These methods are also vulnerable to adversarial attacks, which is a pertinent concern for their reliable deployment in robots and autonomous driving systems. We propose MIMDepth, a method that adapts masked image modeling (MIM) for self-supervised monocular depth estimation. While MIM has been used to learn generalizable features during pre-training, we show how it could be adapted for direct training of monocular depth estimation. Our experiments show that MIMDepth is more robust to noise, blur, weather conditions, digital artifacts, occlusions, as well as untargeted and targeted adversarial attacks.

==> MIMDepth ICRA 2023/files/conclusion.tex <==
\section{Conclusion}
% Depth estimation is an important task for reasoning 3D scene structure from monocular cameras. While most of the existing self-supervised methods focus on the performance on ideal test conditions, we draw attention towards the generalizability and robustness of the network against natural and digital corruptions, occlusions, as well as adversarial corruptions.
We propose a method for adapting masked image modeling (MIM), used until now for self-supervised pre-training of models, into direct training of monocular depth estimation. Our method, MIMDepth, shows improved robustness against noise, blur, weather conditions, digital artifacts, and untargeted and targeted adversarial attacks on depth estimation. While model robustness is often at odds with accuracy, our method is able to maintain comparable depth estimation performance, while also showing improvements in ego-motion estimation. Through ablation studies, we reason about the differences in applying MIM to pre-training and adapting it for depth estimation. We find that blockwise masking (as opposed to random masking) of only the depth estimation network with a relatively lower mask size (than that used for pre-training), and a loss on the complete image (instead of only the masked regions, as used for pre-training) results in more robust depth estimates. We contend that this work could inspire the community to focus on the robustness required in the deployment of depth estimation networks. In the future, such methods could be extended to transformer-based depth estimation with multi-frame input (e.g.~\cite{guizilini2022multi} or overlapping image patches (e.g.~\cite{yang2022depth}). Additionally, MIM could also be adapted for direct training of more downstream tasks.  
% We investigate the application of masked image modelling for training self-supervised monocular depth estimation. While masked image modelling has proven to be useful for pre-training transformers for downstream tasks, its utility for directly training tasks of interest had not been examined. We show that blockwise masking of the depth network during training improves robustness to natural corruptions including uneven illumination and obstructed views of the scene which pose challenges in self-supervised training of the depth estimation networks. Masking during training is also shown to assist in improving robustness to adversarial attacks. We further demonstrate that masked image modelling on the pose network does not benefit depth estimation as the network's context is restricted which reduces its accuracy. Next, we show that unlike masked image modelling for pre-training, masked depth estimation requires a lower level of masking percentage. Finally, also show that using the complete image for loss computation is beneficial compared to using only the masked regions as is the case with masked pre-training. We contend that this work sheds light upon the required robustness in deployment of depth estimation networks and methods to achieve it. In future, such methods could be extended to transformer-based depth estimation with multi-frame input (eg.~\cite{guizilini2022multi} or overlapping image patches(eg.~\cite{yang2022depth}). 

==> MIMDepth ICRA 2023/files/experiments.tex <==
\section{Results}
\label{sec:experiments}
Here, we perform a comparative analysis between the proposed method MIMDepth and existing self-supervised monocular depth estimation methods in terms of their performance on i.i.d. test set, as well as robustness to natural and digital corruptions, occluded views of the scene, and against adversarial attacks. Thereafter, through an ablation study, we resolve the questions posed in Section~\ref{sec:introduction} regarding the mask sampling strategy, size and ratio, as well as the training target for integrating MIM into depth estimation. Finally, we show how integrating MIM into self-supervised monocular depth estimation also results in improved ego-motion estimation on the i.i.d. test set.

\subsection{Settings}
We train the networks on a TeslaV100 GPU for
20 epochs with AdamW optimizer~\cite{loshchilov2017decoupled} at a resolution of 640 × 192 with batchsize 12. The depth and ego-motion encoders are initialized with ImageNet~\cite{deng2009imagenet} pre-trained weights. The learning rate is set at $1e^{-5}$ and decays by a factor of 10 after 15 epochs. 
Unless otherwise stated, the networks are trained on the Eigen-Zhou split~\cite{zhou2017unsupervised} of the KITTI dataset~\cite{geiger2013vision} with 39,810 training, 4424 validation, and 697 test images, respectively. We set the mask size $m_s$, mask ratio $m_r$, aspect ratio $a$ for Algorithm \ref{alg:blockwise_masking_depth} to $16$, $25\%$, and $0.3$, respectively. 

% For MIMDepth, the mask ratio is set at 25\% with a mask size equal to the patch size i.e. $16$. The minimum and maximum block ratios are set to $0.3$ and $1/0.3$ respectively. 
% Single frame, no semantic labels, no synthetic data
\subsection{Robustness}
While multiple works focus on the performance of depth estimation models, deployment in the real world necessitates models that not only perform well in the ideal conditions, but are also robust to various corruptions as well as adversarial attacks.  

To evaluate the robustness, we study the impact
of natural corruptions and adversarial attacks on depth performance against other methods, namely Monodepth2~\cite{godard2019digging}, Packnet~\cite{guizilini20203d}, and MT-SfMLearner~\cite{visapp22} which use 2D convolutions, 3D covolutions, and transformer-based architectures, respectively. We report the robustness of MIMDepth through the average RMSE for models trained with three different seeds.

\subsubsection{Robustness to Natural Corruptions}
The camera used in an autonomous driving vehicle or a driver assistance system can be subject to different corruptions. Particularly, these corruptions can be due to noise (Gaussian, shot, impulse), or blur (defocus, glass, motion, zoom), different weather conditions (snow, frost, fog, brightness) and even digital aberrations (contrast, elastic, pixelation, JPEG). 
Figure \ref{fig:robust_corruptions} compares the different methods on the four types of corruptions, as well as on clean uncorrupted data.
% We observe that while Packnet-SfM has the lowest RMSE on clean data, it is not as robust to natural corruptions. 
Note that the proposed MIMDepth outperforms other methods on clean, noisy, blur, and weather corruptions. 
However, PackNet-SfM is better on digital corruption due to its better performance on pixelated corruption, attributed to its architecture's property of preserving depth details through 3D convolutions. Nevertheless, MIMDepth outperforms it on contrast, elastic, and JPEG digital corruptions. 
% The better performance of Packnet-SfM on pixelation corruption is due to its architecture's property of preserving depth details through 3D convolutions. 
% Also note that MIMDepth is more robust than the baseline method, MTSfMLearner, for all four kinds of corruptions. 
MIMDepth's robustness can be attributed to the higher level of long-range semantic context that is learned by introducing MIM. The impact of a few corruptions on depth estimates is visualized in Figure~\ref{fig:depth}.

% \begin{figure*}[htbp]
% \centering
%     \includegraphics[width=0.3\textwidth]{images/corruptions_heatmap_new.pdf}
%     \includegraphics[width=0.14\textwidth]{images/obstacles_heatmap_new.pdf}
%     \includegraphics[width=0.14\textwidth]{images/obstacles_unmasked_heatmap_new.pdf}
%     \includegraphics[width=0.18\textwidth]{images/untargeted_heatmap_new.pdf}
%   \caption{Robustness to natural and digital corruptions (a), occlusions (center), untargeted adversarial attack (d) } 
% \label{fig:robust}
% \end{figure*}

\begin{figure*}[htbp]
\centering
    \includegraphics[width=0.87\textwidth]{images/heatmaps.pdf}
  \caption{Robustness to natural corruptions, occlusions, and untargeted adversarial attack. Values denote RMSE (m). } 
\label{fig:robust_corruptions}
\end{figure*}

% \begin{figure}[htbp]
% \centering
%     \includegraphics[width=0.8\linewidth]{images/corruptions_heatmap.pdf}
%   \caption{Robustness to natural corruptions } 
% \label{fig:robust_corruptions}
% \end{figure}
% \begin{figure}[htbp]
% \centering
%     \includegraphics[width=0.52\linewidth]{images/obstacles_heatmap.pdf}
%     \includegraphics[width=0.315\linewidth]{images/obstacles_unmasked_heatmap.pdf}
%     \caption{Comparing robustness to occlusions on the complete image and the unmasked regions. } 
% \label{fig:robust_occlusions}
% \end{figure}
% \begin{figure}[htbp]
% \centering
%     \includegraphics[width=0.85\linewidth]{images/untargeted_heatmap.pdf}
%   \caption{Robustness to untargeted attacks} 
% \label{fig:robust}
% \end{figure}

\subsubsection{Occlusion Corruptions}
Monocular depth estimation training requires that the target image is reconstructed using adjacent images. However, due to static as well as dynamic objects, certain regions visible in the target image are occluded in the source image (and vice versa) and cannot be reconstructed. Occlusions are also an important consideration in object-specific depth estimation~\cite{lee2021realtime}. 
% Several strategies have been used to deal with occlusions during training.
However, the role of occlusions has not been studied directly during the test time. Here, we evaluate the impact of occluded context in estimating the depth of objects in the scene. 
% \begin{figure*}[htbp]
% \centering
%   \includegraphics[width=0.4\textwidth]{images/depth_clean.png}
%   \includegraphics[width=0.4\textwidth]{images/depth_obstacle.png}
%   \caption{An example of depth estimation on unobstructed and obstructed views of the scene. } 
% \label{fig:architecture}
% \end{figure*}

\begin{figure*}[t]
\centering
    \includegraphics[width=\textwidth]{images/visualization_depth_filtered.pdf}
  \caption{Examples of depth estimation with different corruptions of the scene.} 
\label{fig:depth}
\end{figure*}

Consequently, we simulate occlusions through modified test sets in which portions of the scene are masked out. Pixels in the occluded region are replaced by the average pixel value of the complete image. In particular, we generate occlusions in the images using blockwise and random masking at the 25\% mask ratio. 
%TODO: To differentiate between masking on test set and training?
% Additionally, we generate a vehicle occlusion test set, where we manually mask out a portion of a single vehicle, for each image in the test set when available. 
% Note that this test directly measures the impact of the introduced masked image modeling within depth estimation.  
% Particularly, we partially mask out vehicles in the scene which are primary target for depth estimation so as to avoid collisions. To do so, we use a semantic segmentation model to identify vehicles, including cars, trucks, motorcycles etc. And mask out  less than 50\% of the object using a square patch of the average color in the region. 

The aim is to evaluate the performance of the depth networks on the unoccluded regions of the scene, as well as to study the direct impact of masked depth estimation in predicting the depth on the complete image. This can also be thought to correspond to scenarios in which only a portion of the target object is visible for object-specific depth estimation. 
Figure ~\ref{fig:robust_corruptions} compares the different methods on the occluded test sets. Occlusions are found to impact depth estimates not only in the masked regions but also in the unmasked regions. We observe that MIMDepth is more robust to occlusions than other methods. By using the global context in a better way, MIMDepth is able to have the best predictions on the unmasked regions and is also able to infer plausible depth for the masked regions. The impact of occlusions on depth estimates for an example image is visualized in Figure~\ref{fig:depth}.

% \begin{figure*}[htbp]
% \centering
%     \includegraphics[width=0.7\textwidth]{images/obstacles_heatmap.pdf}
%   \caption{Robustness to occlusions. } 
% \label{fig:occlusions}
% \end{figure*}

\subsection{Adversarial Attacks}
Adversarial attacks are used to fool networks into making an incorrect prediction through imperceptible changes in input images. These also help to measure the generalizability of the network as the data distribution is altered. We consider two types of adversarial attacks.
% \paragraph{Projected Gradient Descent (PGD)}
For the untargeted attack, we generate adversarial examples following \cite{kurakin2016adversarial} at attack strengths of $\epsilon=\{ 1.0,2.0, 4.0, 8.0, 16.0\}$. The gradients are computed with respect to the training loss $\ell_{depth}$ (see Section \ref{sec:method}) and the perturbations are accumulated over $\min(\epsilon + 4, \lceil1.25\cdot\epsilon\rceil)$ iterations. 
% \paragraph{Symetrically flipped adversarial examples} 
For the targeted attack, we generate adversarial examples that are intended to fool networks into predicting flipped depth estimates~\cite{wong2020targeted}. This attack uses the gradients on the RMSE values corresponding to when the target depths are horizontal or vertical flips of the original prediction. Similar to the PGD attack above, we generate adversarial examples with attack strengths of $\epsilon=\{1.0,2.0, 4.0\}$.

% Adversarial attacks make imperceptible (to humans) changes to input images to create adversarial examples that fool networks. We generate adversarial examples from the i.i.d. test set
% using PGD at attack strength $\epsilon \in \{0.25,0.5,1.0,2.0,4.0\}$. The
% gradients are calculated with respect to the training loss. The perturbation is accumulated over iterations with a step-size of 1. When the test image is from the beginning or end of
% a KITTI sequence, the appearance-based loss is only calculated for the feasible pair of images.

% \begin{figure*}[htbp]
% \centering
%     \includegraphics[width=0.7\textwidth]{images/untargeted_heatmap.pdf}
%   \caption{Untargeted adversarial attacks. } 
% \label{fig:untargeted}
% \end{figure*}

The results of the untargeted adversarial attack are shown in Figure~\ref{fig:robust_corruptions}. The results of horizontal and vertical flipped adversarial attacks on depth estimation are shown in Figure~\ref{fig:targeted}. We note that MIMDepth is the most robust to untargeted and targeted attacks. This can be attributed to the better global context that is learned by adapting MIM to depth estimation. 
% amongst the methods with different architectures. 
% Particularly, we also observe that MIMDepth is more robust than the baseline method, MTSfMLearner, indicating the usefulness of integrating MIM into the depth network for improving its adversarial robustness.

\begin{figure*}[htbp]
\centering
    \includegraphics[width=0.95\textwidth]{images/adv_flip_final.pdf}
  \caption{Targeted horizontal and vertical flip adversarial attacks.} 
\label{fig:targeted}
\end{figure*}


\subsection{Performance}
\begin{figure}[htbp]
\centering
    \includegraphics[width=0.9\linewidth]{images/sota.pdf}
  \caption{Performance of state-of-the-art self-supervised monocular depth estimation methods. The size of the bubble correlates with the accuracy ($\delta<1.25$) for each method (bigger is better).} 
\label{fig:sota}
\end{figure}

It is noted that the accuracy of the model is often at odds with the robustness~\cite{tsipras2018robustness}. Hence, we also compare MIMDepth with other state-of-the-art methods for its performance on the i.i.d. test set in Figure \ref{fig:sota}. For a fair comparison, we consider methods that predict depth only from single images, do not use additional supervised semantic information and train only on KITTI. MIMDepth is able to achieve performance comparable to that of other state-of-the-art methods on both error (RMSE) and accuracy ($\delta < 1.25)$ metrics~\cite{eigen2014depth}. Overall, this shows that integrating MIM into monocular depth estimation improves the robustness of depth estimation while maintaining comparable performance on the i.i.d. test set.

\textit{Model Size and Computational Efficiency:} The expansion in terms of depth model size is limited to the mask token with dimension \emph{d=768} parameters, which is insignificant compared to the baseline depth model size (183 M). Thus, the memory overhead is marginal. Moreover, since image masking is not used during prediction, the inference speed remains the same.  
% The model size is expanded from the baseline only to account for the mask tokens that are equal to the embed dimension of 768 parameters for the depth network. 
% \begin{table}[tb]
% \centering
% \resizebox{\linewidth}{!}{
% \begin{tabular}{|l|c|cc|c|}
% \hline
%  \multirow{2}{*}{\textbf{Methods}} & \multirow{2}{*}{\textbf{Resolution}} & \multicolumn{2}{c|}{\textbf{\cellcolor{red!25}Error$\downarrow$}} & \multicolumn{1}{c|}{\textbf{\cellcolor{blue!25}Accuracy$\uparrow$}} \\ \cline{3-5}
%     &  & Abs Rel & RMSE & $\delta<1.25$ \\ \hline \hline
 
%   % MR
%  CC~\cite{ranjan2019competitive} & 832$\times$256 & 0.140 & 5.326 & 0.826 \\
%   SC-SfMLearner~\cite{bian2019unsupervised} & 832$\times$256 & 0.137 &  5.439 & 0.830 \\
%   Monodepth2 %(ResNet18)
%   ~\cite{godard2019digging} & 640$\times$192 & 0.115 & 4.863 & 0.877 \\
%   SG Depth~\cite{klingner2020selfsupervised} & 640$\times$192 & 0.117 & 4.844 & 0.875 \\
%   PackNet-SfM~\cite{guizilini20203d} & 640$\times$192 & \textbf{0.111} & 4.788 & 0.864  \\
%   Poggi \etal~\cite{poggi2020uncertainty} & 640$\times$192 & \textbf{0.111} & \underline{4.756} & \textbf{0.881}  \\
% % ~\cite{johnston2020self} & 640$\times$192 & \textbf{0.106} & 0.861 & \underline{4.699} & \textbf{0.185} & \textbf{0.889} & \textbf{0.962} & \underline{0.982} \\
% % HR-Depth~\cite{lyu2020hr} & 640$\times$192 & \underline{0.109} & \textbf{0.792} & \textbf{4.632} & \textbf{0.185} & \underline{0.884} & \textbf{0.962} & \textbf{0.983} \\  
%   MT-SfMLearner~\cite{visapp22} & 640$\times$192 & \underline{0.112} & 4.771 & \underline{0.879} \\
%   \textbf{MIMDepth (Ours)} & 640$\times$192 & 0.115 & \textbf{4.743} & 0.875  \\
%   \hline
% \end{tabular}}
% \caption{Quantitative results comparing MiMDepth with existing methods on KITTI Eigen split.}
% \label{tab:depth_table}
% \end{table}

% \begin{table*}[tb]
% \centering
% \resizebox{\textwidth}{!}{
% \begin{tabular}{|l|c|cccc|ccc|}
% \hline
%  \multirow{2}{*}{\textbf{Methods}} & \multirow{2}{*}{\textbf{Resolution}} & \multicolumn{4}{c|}{\textbf{\cellcolor{red!25}Error$\downarrow$}} & \multicolumn{3}{c|}{\textbf{\cellcolor{blue!25}Accuracy$\uparrow$}} \\ \cline{3-9}
%     &  & Abs Rel & Sq Rel & RMSE & RMSE log & $\delta<1.25$ & $\delta<1.25^2$ & $\delta<1.25^3$ \\ \hline \hline
 
%   % MR
%  CC~\cite{ranjan2019competitive} & 832$\times$256 & 0.140 & 1.070 & 5.326 & 0.217 & 0.826 & 0.941 & 0.975 \\
%   SC-SfMLearner~\cite{bian2019unsupervised} & 832$\times$256 & 0.137 & 1.089 & 5.439 & 0.217 & 0.830 & 0.942 & 0.975 \\
%   Monodepth2 %(ResNet18)
%   ~\cite{godard2019digging} & 640$\times$192 & 0.115 & 0.903 & 4.863 & 0.193 & 0.877 & 0.959 & \underline{0.981} \\
%   SG Depth~\cite{klingner2020selfsupervised} & 640$\times$192 & 0.117 & 0.907 & 4.844 & 0.194 & 0.875 & 0.958 & 0.980 \\
%   PackNet-SfM~\cite{guizilini20203d} & 640$\times$192 & \textbf{0.111} & \textbf{0.829} & 4.788 & 0.199 & 0.864 & 0.954 & 0.980 \\
%   \cite{poggi2020uncertainty} & 640$\times$192 & \textbf{0.111} & 0.863 & \underline{4.756} & \textbf{0.188} & \textbf{0.881} & \textbf{0.961} & \textbf{0.982} \\
% % ~\cite{johnston2020self} & 640$\times$192 & \textbf{0.106} & 0.861 & \underline{4.699} & \textbf{0.185} & \textbf{0.889} & \textbf{0.962} & \underline{0.982} \\
% % HR-Depth~\cite{lyu2020hr} & 640$\times$192 & \underline{0.109} & \textbf{0.792} & \textbf{4.632} & \textbf{0.185} & \underline{0.884} & \textbf{0.962} & \textbf{0.983} \\  
%   MT-SfMLearner & 640$\times$192 & \underline{0.112} & \underline{0.838} & 4.771 & \textbf{0.188} & \underline{0.879} & \underline{0.960} & \textbf{0.982} \\
%   \textbf{MIMDepth (Ours)} & 640$\times$192 & 0.115 & 0.852 & \textbf{4.743} & \underline{0.190} & 0.875 & 0.959 & \textbf{0.982} \\
%   \hline
% \end{tabular}}
% \caption{Quantitative results comparing MiMDepth with existing methods on KITTI Eigen split.}
% \label{tab:depth_table}
% \end{table*}



\subsection{Ablation Studies}
Here, we resolve the questions posed in Section~\ref{sec:introduction} about the integration of MIM into self-supervised monocular depth estimation through ablation over different configurations. We use the RMSE on clean input and robustness to occlusion corruptions (for complete image) as the metrics for comparison. 
% We study the utility of applying masked image modelling on the depth and ego-motion network.
% We also compare the use of blockwise and random mask sampling strategies generally used for MIM during pretraining and their impact when applied for training the depth estimation network.   We investigate whether the mask  size and ratios used in MIM for pre-training also work best for MIMDepth. We also analyze if the training target i.e the reconstruction loss for depth estimation should be computed over the complete image or only masked regions after masking is applied. 

% \subsubsection{Mask sampling strategy}
\label{section:results_mask_sampling_strategy}
MIMDepth applies blockwise masking only on the depth network. We have shown that masking the depth network improves the robustness  of the model.
Here, we study the utility of applying MIM also on the ego-motion network. We also compare the use of blockwise and random mask sampling strategies for training the networks.
% We compare the application of the random and blockwise mask strategies on the depth as well as pose networks by evaluating the performance and robustness to different corruptions and adversarial attacks.
From Table \ref{tab:ablation_strategy_obstacles }, we observe that blockwise masking helps the depth estimation network to reduce the mean RMSE over clean and corrupted input. Random masking does not perform as well. This is because block-wise masking is better at inhibiting short-range connections to prevent the network from impainting depth. Furthermore, block-wise masking is more reflective of how specific objects may be occluded rather than random occlusions across the scene. 
We also note that masking the ego-motion network along with the depth network does not improve depth estimation performance on clean data or robustness to occlusions. This could be attributed to the ego-motion network learning the translation and rotation from the shared context of the image pair, which is reduced by masking and is ineffective in improving the dense depth predictions. 
% Since ego-motion estimation network does not make dense prediction and learns to regress pose from channel-wise concatenated images, masking reduces the context 

% This can be attributed to the ego-motion network not learning to make dense predictions. Hence it does not rely upon short range connections across the image that are mitigated by masking.   

%  it will inhibit short range connections and urge the network to learn to predict depth by looking at other objects rather than inpainting depth. It should also help with dealing with occlusion more since objects are often occluded at a stretch.

% corruptions and adversarial attacks as shown in Table . However, masking the pose network does not result in improved robustness when compared against only masking the depth network. This can be attributed to the prediction of translation and rotation not being a dense prediction task. Hence, the network makes the prediction based on the global context of the scene, and masking reduces the available context and hampers the prediction. 

% An exception to this is seen in Table \ref{tab:ablation_strategy_adversarial } where random masing performs better. This can be attributed to the random noise that is added to the images to generate the adversarial examples, which makes MIMDepth trained with random masking better at handling the adversarial attacks. 

% \begin{table*}[]
% \centering
% % \resizebox{\textwidth}{!}{
% \begin{tabular}{|c|c|c|c|c|c|c|}
% \hline
% \multicolumn{1}{|c|}{\textbf{Depth}} & \multicolumn{1}{c|}{\textbf{Ego-Motion}} & \multicolumn{1}{l|}{\textbf{Clean}} & \multicolumn{1}{c|}{\textbf{Noise}} & \multicolumn{1}{c|}{\textbf{Blur}} & \multicolumn{1}{c|}{\textbf{Weather}} & \multicolumn{1}{c|}{\textbf{Digital}}  \\ \hline \hline
% B & -& 4.760 & 5.721 & 5.963 & 5.786 & 5.415  \\
% R & - & 4.777 & 5.901 & 6.064 & 5.784 & 5.424  \\
% B & B & 4.788 & 5.725 & 6.055 & 5.796 & 5.430  \\
% B & R & 4.789 & 5.729 & 6.117 & 5.770 & 5.443 \\
% \hline
% \end{tabular}
% % }
% \caption{Ablation study comparing masking strategies on the depth and pose networks. B refers to blockwise masking. R refers to random masking.}
% \label{tab:ablation_strategy_corruption}
% \end{table*}

% \begin{table*}[]
% % \resizebox{\textwidth}{!}{
% \centering
% \begin{tabular}{|c|c|c|c|c|c|c|}
% \hline
% \multicolumn{1}{|c|}{\textbf{Depth}} & \multicolumn{1}{c|}{\textbf{Ego-Motion}} & \multicolumn{1}{l|}{\textbf{Clean}} & \multicolumn{1}{l|}{\textbf{Bottom}} & \multicolumn{1}{l|}{\textbf{Middle}} & \multicolumn{1}{l|}{\textbf{Left}} & \multicolumn{1}{l|}{\textbf{Right}} \\ \hline \hline
% B & -& 4.760 & 4.791 & 4.823 & 4.891 & 4.781 \\
% R & - & 4.777 & 4.783 & 4.861 & 4.895 & 4.806 \\
% B & B & 4.788  & 4.810 & 4.857 & 4.912 & 4.810  \\
% B & R & 4.789 & 4.799 & 4.859 & 4.929 & 4.814  \\
% \hline
% \end{tabular}
% % }
% \caption{Ablation study comparing masking strategies on the depth and pose networks for Illumination Corruptions. B refers to blockwise masking. R refers to random masking.}
% \label{tab:ablation_strategy_illumination }
% \end{table*}

% \begin{table}[]
% % \resizebox{\textwidth}{!}{
% \centering
% \begin{tabular}{|c|c|c|c|c|c|}
% \hline
% \multicolumn{1}{|c|}{\textbf{Depth}} & \multicolumn{1}{c|}{\textbf{Ego-Motion}} & \multicolumn{1}{l|}{\textbf{Clean}} & \multicolumn{1}{l|}{\textbf{Blockwise}} & \multicolumn{1}{l|}{\textbf{Random}} & \multicolumn{1}{l|}{\textbf{Vehicle}}  \\ \hline \hline
% B & -& 4.760 & 5.570 & 4.983 & 5.261  \\
% R & - & 4.777 & 6.592 & 5.071 & 5.285  \\
% B & B & 4.788  & 5.614 & 5.009 & 5.293   \\
% B & R & 4.789 & 5.579 & 5.010 & 5.297   \\
% \hline
% \end{tabular}
% % }
% \caption{Ablation study comparing masking strategies on the depth and pose networks for Obstacles Corruptions. B refers to blockwise masking. R refers to random masking. Obstacles are also put onto the test images using same strategies or a manually annotated obstacle on a vehicle in the image.}
% \label{tab:ablation_strategy_obstacles }
% \end{table}

\begin{table}[b]
% \resizebox{\textwidth}{!}{
\centering
\begin{tabular}{|c|c|c|c|c|}
\hline
\multicolumn{1}{|c|}{\textbf{Depth}} & \multicolumn{1}{c|}{\textbf{Ego-Motion}} & \multicolumn{1}{l|}{\textbf{Clean}} & \multicolumn{1}{l|}{\textbf{Blockwise}} & \multicolumn{1}{l|}{\textbf{Random}}   \\ \hline \hline
B & -& 4.760 & 5.570 & 4.983  \\ 
R & - & 4.777 & 6.592 & 5.071  \\
B & B & 4.788  & 5.614 & 5.009   \\
B & R & 4.789 & 5.579 & 5.010    \\
\hline
\end{tabular}% }
\caption{Comparing impact of masking strategies for depth and ego-motion networks. B refers to blockwise masking and R refers to random masking. Values denote RMSE (m).}
\label{tab:ablation_strategy_obstacles }
\end{table}

% \begin{table*}[]
% % \resizebox{\textwidth}{!}{
% \centering
% \begin{tabular}{|c|c|c|c|c|c|}
% \hline
% \multicolumn{1}{|c|}{\textbf{Depth}} & \multicolumn{1}{c|}{\textbf{Ego-Motion}} & \multicolumn{1}{l|}{\textbf{Clean}} & \multicolumn{1}{l|}{\textbf{Untargeted}} & \multicolumn{1}{l|}{\textbf{Horizontal Flip}} & \multicolumn{1}{l|}{\textbf{Vertical Flip}}  \\ \hline \hline
% B & -& 4.760 & 5.155 & 8.242 &  7.695 \\
% R & - & 4.777 & 5.148 & 8.099 &  7.625 \\
% B & B & 4.788  & 5.210 & 8.195 & 7.638 \\
% B & R & 4.789 & 5.196 & 8.193 &  7.656  \\
% \hline
% \end{tabular}
% % }
% \caption{Ablation study comparing masking strategies on the depth and pose networks for Adversarial Attacks. B refers to blockwise masking. R refers to random masking.}
% \label{tab:ablation_strategy_adversarial }
% \end{table*}

MIMDepth uses a mask ratio and size of 25\% and 16 respectively. We also compare with the use of a larger mask size or mask ratio in Table \ref{tab:ablation_size_ratio_loss_obstacles}. 
We observe that mask size 16 and mask ratio of 25\% have the lowest mean RMSE over clean and corrupted input. Note that this value is lower than the masking ratio of 40\% used by BEIT~\cite{bao2021beit} or the mask size of 32 used by SimMIM~\cite{xie2022simmim} for pre-training. This can be attributed to the lower information redundancy for depth than that for image reconstruction (e.g. a vehicle with low texture variation and color consistency could have varying relative depth across its body, depending upon its orientation). 
% the masking ratio cannot be as high as used in MIM for pre-training. 

% We  also ablate multiple mask ratios for the mask sizes 16 and 32. 
% We do not test mask sizes below 16 as the mask size has to be a multiple of the patch size. 
% The results for different corruptions and adversarial attacks is summarized in Table \ref{tab:ablation_size_ratio_obstacles }.
% We observe that for both mask sizes, across clean, corrupted, and adversarially perturbed datasets, the average RMSE decreases as the mask size is increased, followed by an increase of the RMSE. 
% For mask size 16, the best performance and robustness is obtained at mask ratio of 25\%, while for the mask size 32, the best performance and robustness is at mask ratio of 15\%. 
% We observe that mask size 16 with mask ratio 25\% has the lowest mean RMSE for all kinds of corruptions and adversarial attacks. Note that this value is lower than the masking ratio of 40\% used by BEIT~\cite{bao2021beit} or even higher used by SIMMIM~\cite{xie2022simmim} and MAE~\cite{he2022masked}. This is due to the information redundancy for depth being lower than that for image reconstruction. Hence the masking ratio cannot be as high as used in MIM for pre-training. 

% \begin{table*}[]
% \centering
% % \resizebox{\textwidth}{!}{
% \begin{tabular}{|c|c|c|c|c|c|c|}
% \hline
% \multicolumn{1}{|c|}{\textbf{Size}} & \multicolumn{1}{c|}{\textbf{Ratio}} & \multicolumn{1}{l|}{\textbf{Clean}} & \multicolumn{1}{c|}{\textbf{Noise}} & \multicolumn{1}{c|}{\textbf{Blur}} & \multicolumn{1}{c|}{\textbf{Weather}} & \multicolumn{1}{c|}{\textbf{Digital}}  \\ \hline \hline
% 16 & 25\% & 4.760 & 5.721 & 5.963 & 5.786 & 5.415  \\
% 16 & 40\% & 4.872 & 5.794 & 6.034 & 5.913 & 5.508  \\
% 32 & 25\% & 4.793 & 5.770 & 5.993 & 5.771 & 5.431  \\
% 32 & 40\% & 4.805 & 5.738 & 6.108 & 5.767 & 5.428 \\
% \hline
% \end{tabular}
% % }
% \caption{Ablation study comparing masking size and ratio of masking on natural corruptions.}
% \label{tab:ablation_size_ratio_corruptions }
% \end{table*}


\begin{table}[b]
\centering
% \resizebox{\textwidth}{!}{
\begin{tabular}{|c|c|c||c|c|c|c|}
\hline
\multicolumn{1}{|c|}{\textbf{Size}} & \multicolumn{1}{c|}{\textbf{Ratio}} & \multicolumn{1}{|c||}{\textbf{Loss}} & \multicolumn{1}{l|}{\textbf{Clean}} & \multicolumn{1}{c|}{\textbf{Blockwise}} & \multicolumn{1}{c|}{\textbf{Random}}  \\ \hline \hline
% 16 & 15\% & Complete & 4.751 & 5.783 & 4.991 \\
16 & 25\% & Complete & 4.760 & 5.570 & 4.983  \\ 
16 & 40\% & Complete & 4.872 & 5.594 & 5.079  \\
32 & 25\% & Complete & 4.793 & 5.612 & 5.016  \\
16 & 25\% & Masked & 4.794	& 5.652	& 5.031 \\
% 32 & 40\% & 4.805 & 5.488 & 5.015  \\
\hline
\end{tabular}
% }
\caption{Comparing the impact of mask ratio, mask size, and training target. Values denote RMSE (m).}
\label{tab:ablation_size_ratio_loss_obstacles}
\end{table}





% \begin{table}[]
% \centering
% % \resizebox{\textwidth}{!}{
% \begin{tabular}{|c|c|c|c|c|}
% \hline
%  \multicolumn{1}{|c|}{\textbf{Ratio}} & \multicolumn{1}{l|}{\textbf{Clean}} & \multicolumn{1}{c|}{\textbf{Blockwise}} & \multicolumn{1}{c|}{\textbf{Random}}  \\ \hline \hline
% % 15\% & 4.751 & 5.783 & 4.991 \\
% 25\% & 4.760 & 5.570 & 4.983  \\
% 40\% & 4.872 & 5.594 & 5.079  \\
% \hline
% \end{tabular}
% % }
% \caption{Comparing impact of mask ratio.}
% \label{tab:ablation_ratio_obstacles }
% \end{table}

% \begin{table}[]
% \centering
% % \resizebox{\textwidth}{!}{
% \begin{tabular}{|c|c|c|c|c|}
% \hline
% \multicolumn{1}{|c|}{\textbf{Size}} & \multicolumn{1}{l|}{\textbf{Clean}} & \multicolumn{1}{c|}{\textbf{Blockwise}} & \multicolumn{1}{c|}{\textbf{Random}}  \\ \hline \hline
% 16  & 4.760 & 5.570 & 4.983  \\
% 32  & 4.793 & 5.565 & 4.993  \\
% \hline
% \end{tabular}
% % }
% \caption{Comparing the impact of mask size.}
% \label{tab:ablation_size_obstacles }
% \end{table}

% \begin{table*}[]
% \centering
% % \resizebox{\textwidth}{!}{
% \begin{tabular}{|c|c|c|c|c|c|c|}
% \hline
% \multicolumn{1}{|c|}{\textbf{Size}} & \multicolumn{1}{c|}{\textbf{Ratio}} & \multicolumn{1}{l|}{\textbf{Clean}} & \multicolumn{1}{c|}{\textbf{Untargeted}} & \multicolumn{1}{c|}{\textbf{Flip Horizontal}} & \multicolumn{1}{c|}{\textbf{Flip Vertical}}  \\ \hline \hline
% 16 & 25\% & 4.760 & 5.155 & 8.242 &  7.695 \\
% 16 & 40\% & 4.872 & 5.328 & 8.563 &  8.087 \\
% 32 & 25\% & 4.793 & 5.194 & 8.475 &  7.932 \\
% 32 & 40\% & 4.805 & 5.317 & 8.516 & 8.039 \\
% \hline
% \end{tabular}
% % }
% \caption{Ablation study comparing masking size and ratio of masking on adversarial attacks.}
% \label{tab:ablation_size_ratio_adversarial }
% \end{table*}

% % \subsubsection{Training target}
% \label{sec:results_mask_trainig_target}
MIMDepth applies the training loss to the complete target image. 
We also compare with applying the loss only on the masked region as used by SimMIM~\cite{xie2022simmim}.  Table~\ref{tab:ablation_size_ratio_loss_obstacles} shows that MIMDepth works better when the loss $\ell_{depth}$ is applied to the entire image. This is due to the training model's focus on learning to predict depth for the complete image, as opposed to the pre-training model's focus on learning representations that only assist downstream tasks at the cost of poor image reconstruction. 


% We evaluate how modifying the loss function when applying masked image modelling impacts the depth predictions. We compare loss functions as applied on the complete image, and only the masked portions. The results are summarized in Table \ref{tab:ablation_strategy_loss_obstacles}. We observe the MIMDepth works better when the loss $\ell_{depth}$ is applied over the complete image. 
% While masked image modelling used in pretraining shows better downstream performance when the loss is applied only on the masked portions~\cite{xie2022simmim}, this effect is not seen when masked image modelling is used to train depth estimation network. This is due to the training model's focus on learning to predict depth for the complete image, as opposed to the pretranining model's focus on learning representations that only assist downstream tasks at the cost of poor image reconstruction. 

% \begin{table*}[]
% \centering
% % \resizebox{\textwidth}{!}
% \begin{tabular}{|c|c|c|c|c|c|c|}
% \hline
% \multicolumn{1}{|c|}{\textbf{Loss}} & \multicolumn{1}{l|}{\textbf{Clean}} & \multicolumn{1}{c|}{\textbf{Noise}} & \multicolumn{1}{c|}{\textbf{Blur}} & \multicolumn{1}{c|}{\textbf{Weather}} & \multicolumn{1}{c|}{\textbf{Digital}} \\ \hline \hline
% \textit{Complete} & 4.760 & 5.721 & 5.963 & 5.786 & 5.415  \\
% \textit{Masked} & 4.794	& 5.816	& 6.021 & 5.815 & 5.172  \\
% \hline
% \end{tabular}
% \caption{Ablation study comparing training using loss function over the complete image against training over only the masked regions.}
% \label{tab:ablation_strategy_loss_natural_corruptions}
% \end{table*}

% \begin{table*}[]
% \centering
% % \resizebox{\textwidth}{!}
% \begin{tabular}{|c|c|c|c|c|c|c|}
% \hline
% \multicolumn{1}{|c|}{\textbf{Loss}} & \multicolumn{1}{l|}{\textbf{Clean}} & \multicolumn{1}{c|}{\textbf{Bottom}} & \multicolumn{1}{c|}{\textbf{Middle}} & \multicolumn{1}{c|}{\textbf{Left}} & \multicolumn{1}{c|}{\textbf{Right}} \\ \hline \hline
% \textit{Complete} & 4.760 & 4.791 & 4.823 & 4.891 & 4.781  \\
% \textit{Masked} & 4.794	& 4.822	& 4.851 & 4.934 & 4.816  \\
% \hline
% \end{tabular}
% \caption{Ablation study comparing training using loss function over the complete image against training over only the masked regions.}
% \label{tab:ablation_strategy_loss_illumination}
% \end{table*}


% \begin{table}[]
% \centering
% % \resizebox{\textwidth}{!}
% \begin{tabular}{|c|c|c|c|c|c|}
% \hline
% \multicolumn{1}{|c|}{\textbf{Loss}} & \multicolumn{1}{l|}{\textbf{Clean}} & \multicolumn{1}{c|}{\textbf{Blockwise}} & \multicolumn{1}{c|}{\textbf{Random}}  \\ \hline \hline
% \textit{Complete} & 4.760 & 5.570 & 4.983   \\
% \textit{Masked} & 4.794	& 5.652	& 5.031    \\
% \hline
% \end{tabular}
% \caption{Comparing impact of training using loss applied over the complete image against only over the masked regions.}
% \label{tab:ablation_strategy_loss_obstacles}
% \end{table}



% \begin{table*}[]
% \centering
% % \resizebox{\textwidth}{!}
% \begin{tabular}{|c|c|c|c|c|c|}
% \hline
% \multicolumn{1}{|c|}{\textbf{Loss}} & \multicolumn{1}{l|}{\textbf{Clean}} & \multicolumn{1}{c|}{\textbf{Untargeted}} & \multicolumn{1}{c|}{\textbf{Horizontal Flip}} & \multicolumn{1}{c|}{\textbf{Vertical Flip}} \\ \hline \hline
% \textit{Complete} & 4.760 & 5.155 & 8.242 &  7.695 \\
% \textit{Masked} & 4.794	& 5.184	& 8.297 &  7.76  \\
% \hline
% \end{tabular}
% \caption{Ablation study comparing training using loss function over the complete image against training over only the masked regions. Measured against adversarial attacks.}
% \label{tab:ablation_strategy_loss_adversarial}
% \end{table*}

\subsection{Impact on Ego-motion estimation Performance}
We additionally evaluate the impact of integrating MIM with depth estimation on the ego-motion estimation predictions. We train MIMDepth on the KITTI odometry split and compare with the baseline MT-SfMLearner in Table~\ref{tab:odom}.  Note that ego-motion predictions on the i.i.d. test set are improved by integrating MIM into the depth network. This can be understood by the use of a common loss for depth and ego-motion networks that is reduced by learning a better context for depth estimation as well as by improving the ego-motion prediction. 

\begin{table}
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{c|cc|cc|}
\cline{2-5}
 & \multicolumn{2}{c|}{09} & \multicolumn{2}{c|}{10} \\ \hline
\multicolumn{1}{|c|}{\textbf{Method}} & $t_{err} (\%)$ & $r_{err} (^{\circ}/100\text{m})$ & $t_{err} (\%)$ & $r_{err} (^{\circ}/100\text{m})$ \\ \hline \hline
% \multicolumn{1}{|c|}{Monodepth2~\cite{godard2019digging}} & 16.332 & 3.552 & 12.086 & 5.110 \\
\multicolumn{1}{|c|}{MT-SfMLearner~\cite{visapp22}} & 9.574 & 2.570 & 13.851 & 5.568 \\
\multicolumn{1}{|c|}{MIMDepth (Ours)} & 6.236 & 2.065 & 8.178 & 3.865 \\ \hline
\end{tabular}}
\caption{Comparison of the performance of ego-motion estimation against the baseline in the KITTI odometry split.}
\label{tab:odom}
\end{table}


==> MIMDepth ICRA 2023/files/introduction.tex <==
\section{Introduction}
\label{sec:introduction}
% Context: Depth estimation for 3d scene understanding application in various scenarios (robotic manipulation, autonomous driving, augmented reality) and challenges (robustness is important) Self-supervision - low cost cameras - digital and other artefacts
\begin{figure*}[htbp]
\centering
  \includegraphics[width=0.88\textwidth, trim=0 0 3.5cm 0, clip]{images/MiMDepth_new.pdf}
  \caption{An overview of 
  Masked Image Modeling for Depth Estimation. The method learns to predict depth from the masked as well as unmasked patches with a better understanding of the global context.} 
\label{fig:framework}
\end{figure*}

Depth estimation is an essential component of vision systems that capture 3D scene structures for applications in mobile robots, self-driving cars, and augmented reality.  Although expensive and power-hungry LiDARs offer high-accuracy depth measurements, the ubiquity of low-cost, energy-efficient cameras makes monocular depth estimation techniques a popular alternative. Traditional methods often estimate depth from multiple views of the scene~\cite{schonberger2016structure}. Instead, deep learning methods have demonstrated depth estimation from a single image. Nevertheless, supervised depth estimation approaches~\cite{lee1907big, yin2019enforcing} require ground truth labels, making it difficult to scale.
% and cannot be deployed to new domains easily. 
On the contrary, self-supervised depth estimation approaches are trained without ground truth labels by using concepts from traditional structure-from-motion and offer the possibility of training on a wide variety of data~\cite{chawlavarma2021multimodal, guizilini20203d}. However, the deployment requires a focus on the generalizability and robustness of models beyond performance under ideal conditions~\cite{chawlavarma2022adversarial}.  


% Gap: MTSfM showed that robustness is higher. But limited focus on robustness in literature. All chase accuracy in ideal conditions. 
Recently, MT-SfMLearner~\cite{visapp22} showed that the transformer architecture for self-supervised depth estimation results in higher robustness to image corruptions as well as against adversarial attacks.  This is attributed to transformers utilizing the global context of the scene for predictions, unlike convolutional neural networks that have a limited receptive field. However, most research in self-supervised monocular depth estimation focuses primarily on achieving excellent performance on the independent and identically distributed (i.i.d.) test set.  It is assumed that the images are free from noise (e.g. Gaussian) and blur (e.g. due to ego-motion or moving objects in the scene), have clear daylight weather, and are without digital artifacts (e.g. pixelation).  Even for the task of object-specific depth estimation~\cite{lee2021realtime}, it is assumed that the objects are without occlusions. Finally, the robustness of methods against adversarial attacks is not considered, which is a pertinent concern for safety while deploying deep learning models.  

% Clue: Masked Image Modeling from pretraining. inductive biases. Identify similarities. 
Since the performance and robustness of the models are determined by the learned representations, influencing the encoding of features could lead to more robust estimations. We hypothesize that integrating Masked Image Modeling (MIM) into the training of depth estimation would result in learning features that make the model more robust to natural and digital corruptions as well as against adversarial attacks, by modeling the global context in a better way. MIM is a technique that has been used until now for self-supervised representation learning in pre-training of image transformers~\cite{bao2021beit, xie2022simmim,he2022masked,wei2022masked}.
% MIM has shown tremendous results in downstream fine-tuning for tasks like image classification and segmentation~\cite{bao2021beit, xie2022simmim, he2022masked, wei2022masked}. 
% Following the introduction of masked \textit{language} modeling (MLM) in BERT~\cite{kenton2019bert}, MIM  has gained popularity for self-supervised representation learning in image transformers with tremendous results in downstream tasks~\cite{bao2021beit, xie2022simmim, he2022masked, wei2022masked}. 
MIM pre-training involves masking a portion of image patches and then using the unmasked portion to predict the masked input~\cite{xie2022simmim, he2022masked} or its features~\cite{bao2021beit, wei2022masked}. It models long-range dependencies and focuses on the low-frequency details present in the images.
% resulting in improved representations through the global context. 
However, when pre-trained models are fine-tuned for downstream training, the general features that were learned could possibly be overwritten.  Instead, adapting MIM for direct training of a task, such as depth estimation, could lead to richer learned representations that make the model more robust and generalizable. 
% However, these rich representations may be overwritten when training on a downstream task.
% However, MIM has not been utilized in direct training of a task such as depth estimation, where the richer representations could make the model more robust and generalizable.  

% Contribution: Identify gaps (questions to be answered / hypothesis i.e. differences)
% We hypothesize that integrating MIM into depth estimation would result in learning features that make depth estimation more robust to natural and digital corruptions as well as adversarial attacks, by modeling the global context in a better way. 
While both MIM and depth estimation are self-supervised methods, they differ in how they are trained. MIM, used in pre-training of a network, learns by reconstructing the input image generally passed through an autoencoder. Instead, the self-supervised depth estimation network is trained along with a self-supervised ego-motion estimation network, whose output is used to synthesize adjacent images in the training set via the perspective projection transform~\cite{zhou2017unsupervised}.  
Thus, applying MIM to depth estimation requires different considerations than its use for pre-training. Here, we examine the following questions:
\begin{itemize}
    \item Would integrating MIM to the depth and/or ego-motion estimation networks result in improved robustness of depth estimation?
    % \item Would integrating MIM to the ego-motion estimation network result in improved robustness of depth estimation?
    \item  MIM has been shown to work well with either blockwise masking~\cite{bao2021beit}, or random masking with high mask size~\cite{xie2022simmim}. Which masking strategy would work better for depth estimation?
    % \item  MLM utilizes a mask ratio of 15\%~\cite{kenton2019bert}  
    \item MIM pre-training uses a relatively high mask ratio and mask size~\cite{bao2021beit, xie2022simmim, he2022masked} due to more information redundancy in images than in sentences. Would the high mask ratio or high mask size used for MIM pre-training be suitable for integrating it into depth estimation? 
    \item MIM has been shown to result in better features for downstream tasks when its loss is applied only to masked regions~\cite{xie2022simmim}. Would similarly applying the loss on only the masked regions result in a more robust depth estimation?
\end{itemize}

With our proposed method MIMDepth, we demonstrate that applying blockwise masking with a relatively lower mask ratio (than MIM pre-training) only to the depth estimation network, with a loss on the complete image, results in improved robustness to natural and digital corruptions, occlusions, as well as untargeted and targeted adversarial attacks.
% MIMDepth maintains a competitive performance on the i.i.d. test set while improving its performance on the i.i.d
It is additionally found to improve the performance of the ego-motion estimation network, while maintaining a competitive performance of the depth estimation network on the i.i.d. test sets. 




% % Context: Representation learning and masked image modeling and differences between language and vision masking. Gap: Only evaluated on pre-training
% The success of deep learning models 
% in scene understanding tasks 
% is based upon their ability to learn better representations, reflecting an improved semantic understanding of the input. Following the introduction of masked \textit{language} modeling in BERT~\cite{kenton2019bert}, masked \textit{image} modeling (MIM)  has also gained popularity for self-supervised representation learning in image transformers with tremendous results in downstream tasks~\cite{bao2021beit, xie2022simmim, he2022masked, wei2022masked}.
% %  Following the advent of Transformers~\cite{vaswani2017attention}  for natural language processing, BERT~\cite{kenton2019bert} introduced masked language modeling for self-supervised representation learning. Similar success has has been seen for pre-training image transformers~\cite{} through masked image modeling. 
% In general, masked signal modeling involves masking a portion of the words or image patches, and then using the unmasked signals to predict the masked input~\cite{xie2022simmim, he2022masked} or its features~\cite{bao2021beit, wei2022masked}. In practice, this implies processing non-overlapping tokenized  inputs~\cite{dosovitskiy2020vit,vaswani2017attention}, of which some have been replaced with special mask tokens.  
% % Since the masked signals can be thought of as noise,  masked image modeling is also seen in the context of denoising masked autoencoders~\cite{}.  
% While masked image modeling has been used to pre-train networks with large unlabelled data for a variety of downstream tasks, it has not been applied directly for training a relevant task of interest. 



% % Modern scene understanding tasks utilize deep learning models that have a hierarchy of representations to map the input to the output. Their success lies in their ability to learn  higher-level abstract concepts which reflect a semantic understanding of the input. 
% % The data used for training as well as the architecture of the network introduces inductive biases in the model influencing its capability to learn these concepts.
% % Often networks are pre-trained on a large dataset such as ImageNet before finetuning for a downstream task. While such pre-training often uses supervised learning with labeled data, masked signal modeling has been used for pre-training language and vision transformers in a self-supervised fashion with tremendous results. Nevertheless, the impact of masked signal modeling beyond pre-training on application tasks has not been studied. 

% % Content: Masked Image Modelling for Depth Estimation 
% % Depth estimation and image reconstruction
% % Use of transformers
% % Subfield gap: how would masked image modelling apply and what are the differences expected

% Self-supervised monocular depth estimation is one such task of interest in 3D scene understanding. It is trained in parallel with a monocular ego-motion estimation network. 
% % Learned together with ego-motion estimation, the training paradigm consists of using the outputs of the two networks for reconstruction of neighboring images in videos~\cite{}.
% Specifically, the monocular depth of a target frame and its relative ego-motion with the neighboring image frame is used to warp the neighboring frame to reconstruct the target frame.
% Thereafter, analogous to the loss for the autoencoding-based MIM methods~\cite{xie2022simmim, he2022masked}, the loss between the reconstructed target image and the original target image is used to train the networks.
% % to train the depth and ego-motion estimation networks simultaneously.
% Since the image is reconstructed from a neighboring frame, the illumination changes and obstructed views of the objects present a challenge to self-supervised depth training~\cite{bian2021unsupervised, guizilini20203d}, which existing methods deal with in various ways.  
% Most of the existing self-supervised monocular depth estimation networks are nevertheless based on convolutional neural networks~\cite{bian2021unsupervised, godard2019digging, lyu2020hr}, which are generally not capable of receiving tokenized inputs~\cite{visapp22} that are needed for MIM.  

% % Until recently, most of the depth estimation models were based on Convolutional Neural Networks which don't easily allow for the use of mask tokens with positional embeddings. However, the introduction of transformers for self-supervised monocular depth estimation, has provided an opportunity to investigate 



% % Monocular depth and ego-motion estimation, learned simultaneously in a self-supervised manner are two of the key tasks for 3D scene understanding in robotics. Occlusions and lack of robustness to illumination changes is considered a challenge for these regression tasks.  Such a task can be utilized to investigate the impact of masked image modeling  during training on performance and robustness of the models.  Masked signal modeling in image transformers occludes patches of image tokens during training using a blockwise or random masking strategy during training.  Their use focuses on reducing the learning of high-frequency redundant information in images. While this has been helpful in learning representations that assist in recognition tasks, their use for regression tasks remains to be evaluated. 

% % Clues: Mask strategy, size, ratio, loss function related untested hypothesis. and link to robustness
% \cite{visapp22} recently proposed MTSfMLearner, a transformer-based depth and ego-motion estimation method which resolves this precondition to utilize MIM. 
% % allowing the application of MIM.
% % The primary objective of using MIM has been to learn representations that model improved semantic relationships in the encoder. 
% As applied on pre-training, MIM leads to improvements in learned representations via modeling long-range dependencies, focusing on the low-frequency details present in the images~\cite{bao2021beit}. 
% It has been shown that a blockwise masking strategy~\cite{bao2021beit}, or even random masking with a high mask size or masking ratio~\cite{xie2022simmim} assists in this objective.
% These are necessary due to images containing low-level information which is highly spatially redundant, allowing information about the masked patches to be recovered using photometrically similar nearby patches. Furthermore, the primary objective of MIM in pre-training is to have a good performance on downstream tasks, and not the quality of prediction of masked image patches or their features. It has been shown that computing the loss over the masked patches rather than the complete reconstructed input can lead to better downstream performance~\cite{xie2022simmim}. 
% In contrast, our focus is on directly regressing pixelwise depth, wherein nearby patches that are photometrically similar can have different depths. 
% Therefore, the level of information redundancy in an image to model a depth map is lower than that to reconstruct the corresponding image.
% Accordingly, we hypothesize that the observations about mask sampling strategy as well as the target loss for masked depth estimation will differ from those when MIM is applied to pre-training.  We also hypothesize that MIM would help learn features for depth estimation that may be robust to occluded views and uneven illumination. 
% %  However, applying MIM for direct depth estimation should also lead to different conclusions about the training target. 
% % While MIM is shown to perform better when the loss is computed over only the masked regions, depth estimation will have no such benefit.
% Overall, it remains to be explored how MIM could be effectively applied to regressing monocular depth, and what are its potential benefits.  

% % Ego-motion estimation on the other hand directly predicts the translation and rotation from a pair of images. This requires looking the global relations across the image pair patches. Thus, we posit that MIM on the pose network won't be  


% % There are several differences between applying masked signal modeling to language, images, and potentially depth estimation. The input to the language model are words which are discrete and semantically rich, unlike visual signals which are continuous and contain low-level information. 


% % MTSfMLearner showed that the global receptive field of transformers assists in improving the robustness to natural corruptions and adversarial attacks while maintaining competitive performance.


% % low level - ok to reconstruct pixels, can it capture features to predict depth
% % level of redundancy and locality of information
% % short range and long range 



% % Applying masked image modeling for training monocular depth and ego-motion estimation networks would urge the models to learn from different regions and features in the image, breaking the shortcuts that are generally learned. While transformer models focus on the global context of the scene and do not have inductive bias to local proximity unlike Convolutional Neural Networks, use of masking in depth estimation would further help break the short range dependencies.  We hypothesize that masked image modeling will also help the networks deal with occlusions in the real world and also improve the robustness of the models to natural corruptions and adversarial attacks. 

% % % Contributions: We use MTSfMLearner. Compare on KITTI, with CNN, Packnet 3d convolutions, transformer architechtures

% We propose MIMDepth, a framework for masked depth estimation following the principles of masked image modeling. We adapt the depth estimation network in MTSfMLearner for this purpose, and demonstrate that MIMDepth achieves higher robustness to natural corruptions and adversarial attacks than contemporary depth estimation methods while maintaining competitive performance on the Eigen-Zhou~\cite{zhou2017unsupervised} split of the KITTI dataset~\cite{geiger2013vision}.  We also examine the various configurations of the masked depth estimation vis-a-vis contemporary MIM approaches including the mask strategy, mask size and ratio, as well as the target loss function. For masked depth estimation, we find that blockwise masking is better than random masking, masking on the ego-motion network is not beneficial compared against the masking of only the depth network, the best mask size and ratio are lower than that for MIM pre-training, and that applying the loss over the complete reconstructed image leads to better results. We hope that our results will motivate further research in improving the robustness of depth estimation as necessary for safe deployment of these models. 
% % We find that the observations about the best configuration of masking depth estimation network differ from the  




% % We study the role of masked signal modelling o on transformer-based monocular depth estimation. Particularly, we build upon  Monocular Transformer Structure-from-Motion Learner (MT-SfMLearner) considering different masking strategies, mask sizes, and mask ratios, application of loss functions. We evaluate the performance on the Eigen-Zhou split of the KITTI dataset, and also measure the robustness of the model against corruptions due to noise, blur, weather conditions, and digital effects. Additionally, we measure the robustness to uneven illumination and obstructed views in the images, both of which are challenges for training depth estimation networks. We also evaluate the generalization performance through untargeted and targeted adversarial attacks. We demonstrate that masked signal modelling assists monocular depth estimation be more robust while maintaining competing performance. 

% % \begin{enumerate}
% % \item Blockwise masking will work better for depth as it will inhibit short range connections and urge the network to learn to predict depth by looking at other objects rather than inpainting depth. It should also help with dealing with occlusion more since objects are often occluded at a stretch. 
% % \item Pose estimation looks at a global context, and hence it does not rely upon short range connections across one single image. Therefore blockwise should have no benefit over random. 
% % (Ideally we should show on odom split training (perhaps we can do after the configuration has been selected). Alternative: Pose estimation already looks at global context. Masking of any kind will reduce the context available and will not help. 
% % \item Loss over the masked and unmasked portions together is better than just over the masked or just over the unmasked regions. While SimMIM suggests that using the masked region alone helps representation learning for downstream tasks, using both should help the dense prediction task of depth estimation and the regression task for pose estimation.
% % \item Higher mask size would help improve robustness of the pose network as it looks as the global context of the scene.  
% % \item The ideal mask ratio for MIM training is lesser than that used for MIM pretraining. 
% % \item Higher mask ratio and medium mask size are better than higher mask size and medium mask ratio because it acts as partially occlusion for objects in the scene. 
% % \end{enumerate}

% % Our results demonstrate...


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % The deep learning community is experiencing a trend of unifying methodologies for solving problems
% % in different areas, such as language, vision, speech, and more. For architectures, Transformers [67]
% % have been successfully introduced into computer vision [18] and established as a general building
% % block in both language and vision. For self-supervised representation learning, the denoising/masked
% % autoencoding methodology in BERT [15] has been shown effective on learning visual representations from images [31].

% % no extra problem-specific tokenizer. masking ratio (i.e., percentage of removed tokens) in masked
% % autoencoding methods is related to the information redundancy of the problems. For example, natural
% % images are more information-redundant than languages and thus the optimal masking ratio is higher
% % (e.g., than BERT [15]). 


% % Over the years vision transformers have shown the ability to rival deep convolution in the field of computer vision by focusing on the similarity between its own elements within an image to improve the semantic information of the representation

% % One essential difference between vision and language is
% % that vision has no pre-existing vocabulary to shape the prediction task into a well-defined classification problem. In
% % contrast, the raw spatiotemporal visual signal is continuous
% % and dense posing a major challenge to masked visual prediction. One immediate solution is to imitate the language
% % vocabulary by building a visual vocabulary that discretizes
% % frame patches into tokens, as explored in BEiT [2, 58].
% % However, this requires an external tokenizer which can be
% % limited in compute-intensive video understanding scenario.


% % The solutions, based on autoregressive language
% % modeling in GPT [47, 48, 4] and masked autoencoding in
% % BERT [14], are conceptually simple: they remove a portion
% % of the data and learn to predict the removed content

% % The idea of masked autoencoders, a form of more general denoising autoencoders [58], is natural and applicable
% % in computer vision as well

==> MIMDepth ICRA 2023/files/method.tex <==
\section{Method}
\label{sec:method}

% - learnable mask tokens
% - ssl and reconstruction
% - texture of depth similar but depth different (expts)
% - change context image to source image (relate to diagram)
% - order: depth, masking, connection with hypothesis

% \begin{figure*}[htbp]
% \centering
%   \includegraphics[width=0.8\textwidth, trim=0 0 3.5cm 0, clip]{images/MiMDepth_new.pdf}
%   \caption{An overview of 
%   Masked Image Modeling for Depth Estimation. The network learns to predict depth from the masked as well as unmasked patches by understanding the global context better.} 
% \label{fig:framework}
% \end{figure*}

We propose MIMDepth, a method for masked self-supervised monocular depth estimation (see Figure \ref{fig:framework}) that integrates masked image modeling (MIM) into self-supervised monocular depth estimation. MIMDepth trains the depth estimation network by masking a portion of the input,  while the network learns to predict complete pixelwise depth from the partial observations, including for the masked portions. Hereafter, we elaborate upon the components of the method.

\subsection{Self-supervised Monocular Depth Estimation} We use MT-SfMLearner~\cite{visapp22} as the baseline monocular depth estimation method, which we briefly summarize here. 
Similar to other self-supervised methods, it trains depth and ego-motion estimation networks simultaneously. The training input to the networks is a set of consecutive image triplets $\{I_{-1}, I_0, I_1\}$ from a video. The depth network is trained to output pixel-wise depth for the target image $I_0$, while the ego-motion estimation network is trained to output relative translation and rotation between the image pairs $\{I_{-1}, I_0\}$ and $\{I_0, I_1\}$.  Note that for the ego-motion estimation network, the input pair of images is concatenated along the channel dimension. Both the depth and ego-motion estimation networks utilize a transformer-based encoder DeiT-Base~\cite{touvron2021training} which processes the tokenized inputs at constant resolution. 

The predicted depth and ego-motion are linked together via the perspective projection transform for a given set of camera intrinsics $K$, through which the source images $I_{-1}$ and $I_1$ are warped to synthesize the target image $\hat{I}_0$.  Both the depth and the ego-motion estimation networks are trained simultaneously using a common loss $\mathcal{L}_{depth}$ between $\hat{I}_0$ and $I_0$, which is a weighted sum of two losses. 
First is the appearance-based photometric loss between the original and the synthesized target image, $\mathcal{L}_{photo}$. The photometric loss is itself composed of a structural similarity $(\mathcal{L}_\text{SSIM})$ loss~\cite{wang2004image} and an $\ell_1$ distance loss between the images.  Second is a smoothness loss on the depth output, $\mathcal{L}_\text{smooth}$, for regularization in low-texture portions of the scene. Therefore, 
\begin{equation}
    \mathcal{L}_{depth} = \lambda_1 \cdot \mathcal{L}_\text{SSIM} + \lambda_2 \cdot \ell_1 + \lambda_3 \cdot \mathcal{L}_\text{smooth},
\end{equation}
where $\lambda_1$, $\lambda_2$, and $\lambda_3$ are the hyperparameter weights for the losses.

\subsection{Integrating Masked Image Modeling}
Our method MIMDepth, integrates MIM with self-supervised monocular depth estimation for masked self-supervised depth estimation. While MIM in pre-training applies masking for the network that reconstructs the image, we could mask the input to the depth or the ego-motion estimation networks. 
The input to the depth estimation network is a single image, which is converted into non-overlapping patches with token and position embeddings. 
For integrating MIM with the depth network, we use a mask generator to sample the patch indexes to be masked. The method for mask generation is described in Algorithm~\ref{alg:blockwise_masking_depth}. 
A block with a random aspect ratio is repeatedly selected to be masked in the image until the required mask ratio is achieved.  The indexes to be masked are replaced with learnable masked token embeddings, which are initialized as Gaussian noise. 

We use a blockwise masking strategy similar to BEIT~\cite{bao2021beit}, but we do not use any dVAE to generate targets. We use a mask ratio of 25\% which is higher than that used in MLM but less than that used in MIM pre-training. This is due to the lower information redundancy in the depth of objects than in their texture. As an example, a gray color car would have similar texture across the pixels, but its depth would vary depending upon how it is oriented with respect to the camera. The network is trained to directly predict the depth for the complete image from the partially masked input. However, we do not apply masking to the ego-motion network, as it does not improve depth estimation (see Section~\ref{sec:experiments}). 

SimMIM~\cite{xie2022simmim} shows that it is better to learn to predict over the masked patches rather than the complete image in order to pre-train representations that assist in downstream tasks.   This is because training the network on the complete image would waste learning capability on the reconstruction quality of unmasked portions. However, with MIMDepth, the objective is to directly learn pixel-wise dense prediction including the unmasked portions. Hence, we apply the loss $\mathcal{L}_{depth}$ to the complete target image. 

\begin{algorithm}[t]
\footnotesize
\DontPrintSemicolon
\SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
\SetKwFunction{Random}{random}
\SetKwFunction{Gaussian}{$\mathcal{N}$}
\SetKwFunction{repeat}{repeat}

\SetKwRepeat{Do}{do}{while}

\SetKwData{h}{h}
\SetKwData{w}{w}
\SetKwData{aspect}{aspect}
\SetKwData{MaskRatio}{mask\_ratio}
\SetKwData{MaskSize}{mask\_size}
\SetKwData{NumPatches}{num\_patches}
\SetKwData{MaskRatio}{mask\_ratio}

\Input{unmasked tokens $x_u$ \\
% \MaskSize \\
mask size $m_s$ \\
% \MaskRatio \\ 
mask ratio $m_r$ \\
% image shape (\h $\times$ \w)
image shape ($h \times w$) \\ 
block aspect ratio $a$
} 

\Output{masked tokens $x_m$}
\BlankLine

% \NumPatches $\leftarrow$ $\frac{\h \times \w}{\MaskSize^2}$ \\
$n \leftarrow (h \times w) / m_s^2$  \tcp*[0]{num maskable patches} 
$M \leftarrow$ [] \tcp*[0]{initialize mask}
% \Do{$|M| <$ \MaskRatio $\times$ \NumPatches}{
\Do{$|M| < m_r \times n$}{
% s $\leftarrow$ \Random(\MaskSize, \MaskRatio $\times$ \NumPatches $- |M|$) \tcp*[0]{Select Block size} 
$s \leftarrow \Random(m_s, m_r \times n - |M|$) \tcp*[0]{select block size}
% r $\leftarrow$ \Random(\aspect, \aspect$^{-1}$), $ \aspect < 1$ \tcp*[0] {Select Block aspect ratio} 
$r \leftarrow \Random(a, a^{-1}),  a < 1$ \tcp*[0]{select block aspect ratio} 
% a $\leftarrow$ $\sqrt{s \cdot r}$; b $\leftarrow$ $\sqrt{s/r}$\\
% y $\leftarrow$ \Random(0, $\h - \sqrt{s \cdot r}$); x $\leftarrow$ \Random(0, $\w - \sqrt{s/r}$)\\
$x \leftarrow \Random(0, w - \sqrt{s/r}$) ; $y \leftarrow \Random(0, h - \sqrt{s \cdot r}$) \\
$M_{block} \leftarrow \{ (i,j): i \in [y, y+\sqrt{s \cdot r} ], j \in [x, x+\sqrt{s/r}]  $\} \\
% $M \leftarrow M \cup \{ (i,j): i \in [y, y+\sqrt{s \cdot r}], j \in [x, x+\sqrt{s/r}]  $\} \tcp*[0]{add block to mask}
$M \leftarrow M \cup M_{block}$ \tcp*[0]{add block to mask}
}
% $M$ = \repeat($M$, $\h//\MaskSize$, $\w//\MaskSize$) \tcp*[0]{Repeat mask to match the transformer patch size}
$M \leftarrow M.\repeat(\lfloor h/m_s \rfloor, \lfloor w/m_s \rfloor$) \tcp*[0]{repeat mask to match the transformer patch size}
% $x_m$ $\leftarrow$ $x_u \times (1-M) $ + \Gaussian$(0, 0.02) \times M$ \tcp*[0]{Generate masked tokens}
$x_m \leftarrow x_u \times (1-M)  + \Gaussian(0, \delta) \times M$ \tcp*[0]{generate masked tokens}
\KwRet{$x_m$}
\caption{Blockwise Masking for Depth Estimation Network}
\label{alg:blockwise_masking_depth}
\end{algorithm}

% For generating the learnable masked token embeddings, we utilize a Masking Generator, with its method as formulated in Algorithm \ref{alg:blockwise_masking_depth}. The mask size and ratio are set to 16 for MTSfMLearner (equal to its patch size) and 25\%, respectively. Note that this masking ratio is less than that used by \cite{bao2021beit} for MIM during pretraining. 
% Accordingly, the  token embeddings at the sampled locations are replaced with the learnable masked tokens which are initialized as Gaussian noise. 

%%%%%%%








% % MIMDepth is composed of three components, namely, the transformer-based monocular depth estimation approach, the mask sampling strategy, and the training target.  We hereafter elaborate upon these components.

% % Such methods,generally used in pre-training of language and image models introduce non-local inductive biases into the network to assist in downstream tasks. However, we demonstrate how these can be incorporated into the training protocol of self-supervised depth estimation to improve the robustness of the models to various corruptions as well as adversarial attacks. 
% \subsection{Self-supervised Depth Estimation Approach}
% As discussed earlier, recent masked image modeling methods require the ability to receive and process tokenized inputs. Therefore, we utilize a transformer-based method MTSfMLearner~\cite{visapp22} for monocular depth estimation in our framework.  Here we provide a brief summary of this method and how we integrate masked image modeling into it. Both the depth and ego-motion estimation networks utilize a transformer-based encoder DeiT-Base~\cite{touvron2021training} which processes the tokenized inputs at a constant resolution. As shown in Figure \ref{fig:framework}, the input to the depth estimation network is a single image which is converted into non-overlapping patches with token and position embeddings. 



% Similar to other self-supervised methods, MTSfMLearner trains depth and ego-motion estimation networks simultaneously. The training input to the network is a set of consecutive image triplets $\{I_{-1}, I_0, I_1\}$ from a video. The depth network is trained to output pixewise depth for the target image $I_0$, while the ego-motion estimation network is trained  to output relative translation and rotation between the image pairs $\{I_{-1}, I_0\}$ and $\{I_0, I_1\}$. The predicted depth and ego-motion are linked together via the perspective projection transform for given set of camera intrinsics $K$, through which the context images $I_{-1}$ and $I_1$ are warped to synthesize the target image.  
% Note that while MTSfMLearner allows to predict the camera intrinsics along with the depth and the pose, we do not use that functionality in this method for a more direct comparison with other approaches. 

% Both the depth and ego-motion estimation networks utilize a transformer-based encoder DeiT-Base consisting of 12 transformer layers with multi-head self-attention~\cite{touvron2021training} which processes the tokenized inputs at a constant resolution. As shown in Figure \ref{fig:framework}, the input to the depth estimation network is a single image which is converted into non-overlapping patches with token and position embeddings. Simultaneously, the mask generator is used to sample the patch indexes which will be masked. Accordingly, the  token embeddings at the sampled locations are replaced with the learnable masked tokens which are initialized as Gaussian noise. The masking process is elaborated further in the next subsection. The input to the ego-motion estimation network is a pair of images concatenated along the channel dimension, with its embedding layer repeated accordingly. However, we do not apply masking to the ego-motion network.  The reasons for this are substantiated in section \ref{section:results_mask_sampling_strategy}. 

% % \subsection{Background: Self-supervised Depth and Pose Estimation}
% % Self-supervised depth and pose estimation networks are trained simultaneously as auxiliary tasks to the main objective of image reconstruction through neighboring frames in videos. For a series of consecutive images in a video, the depth network is trained to output dense pixelwise depth for each image, while the pose network is trained to predict relative ego-motion (rotation and translation) between two consecutive images. The predicted depth and relative ego-motion are linked together via the perspective projection transform. This is used to synthesize the adjacent target image by using the depth of the given source image and the relative translation and rotation between them. The photometric error between the synthesized target image the original target image is used as a loss for training. 

% % The networks are trained using the appearance-based photo-
% % metric loss between the real and synthesized target images,
% % as well as a smoothness loss for depth regularization in low
% % texture scenes [4]. Following [4], [27], we use auto-masking
% % (M) to disregard the temporally stationary pixels in the image
% % triplets. The total appearance-based loss is calculated by
% % upscaling the predicted depths from intermediate decoder
% % layers to the input resolution

% % \begin{figure*}[htbp]
% % \centering
% %   \includegraphics[width=\textwidth, trim=0 0 3.5cm 0, clip]{images/MiMDepth_new.pdf}
% %   \caption{An overview of 
% %   Masked Image Modeling for Depth Estimation. The network learns to predict depth from the masked as well as unmasked patches by understanding the global context better.} 
% % \label{fig:framework}
% % \end{figure*}


% \subsection{Mask Sampling Strategy}
% For generating the learnable masked token embeddings, we utilize a Masking Generator, with its method as formulated in Algorithm \ref{alg:blockwise_masking_depth}. The mask size and ratio are set to 16 for MTSfMLearner (equal to its patch size) and 25\%, respectively. Note that this masking ratio is less than that used by \cite{bao2021beit} for MIM during pretraining. This is substantiated in section \ref{section:results_mask_sampling_strategy}. 

% Specifically, we utilize the blockwise masking strategy as proposed in \cite{bao2021beit}. This strategy prevents the network from focusing on short-range dependencies and from inferring depth from those of nearby pixels. In this method, the masked positions are computed over multiple iterations, with each iteration masking a rectangular block within the patchified-image. The masked block in each iteration may overlap with the previously masked regions. This process is repeated until the desired percentage of patches are masked. We allow the mask size to be a multiple of the transformer patch size. Therefore, the generated mask is repeated to match the transformer patch size if the mask size is larger. The output of this method is binary mask $M$.

% Finally, the mask is utilized to replace the corresponding token embedding with Gaussian noise. This is illustrated in Figure \ref{fig:framework}. Note that we use the same standard deviation of $0.02$ as is used by \cite{bao2021beit}.

% The depth network then learns to predict depth with missing context in the scene. The regression of pixelwise depth aligns with the continuous nature of the ordered visual signals, yet is a more complex task than that of image reconstruction. 



% \subsection{Training target}
% \label{sec:training_target}
% While we use the blockwise masking strategy as described in \cite{bao2021beit}, we do not use any discrete VAE to generate the targets. 
% Both depth and pose estimation networks are trained simultaneously using a common loss $\mathcal{L}_{depth}$, which is a weighted sum of two losses. 
% First is the appearance-based photometric loss between the original and the synthesized target image, $\mathcal{L}_{photo}$. The photometric loss is itself composed of a structural similarity $(\mathcal{L}_{SSIM})$ loss and an $\ell_1$ loss between the images.  Second is a smoothness loss on the depth output for regularization in low-texture portions of the scene, $\mathcal{L}_{smooth}$. Therefore, 
% \begin{equation}
%     \mathcal{L}_{depth} = \lambda_1 \cdot \mathcal{L}_{SSIM} + \lambda_2 \cdot \ell_1 + \lambda_3 \cdot \mathcal{L}_{smooth},
% \end{equation}
% where $\lambda_1$, $\lambda_2$, and $\lambda_3$ are the weights for the losses respectively. 
% % This loss is a weighted sum of the appearance-based photometric loss between the original and the synthesized target image, as well as a smoothness loss on the depth output for regularization in the low-texture portions of the scene. 

% For pre-training, SimMIM~\cite{xie2022simmim} shows that it is better to learn to predict over the masked patches rather than the complete image in order to learn representations that assist in downstream tasks.   This is because the network would waste learning capability on reconstructing a better image. However, with MIMDepth, the objective is to directly learn pixelwise dense prediction. Hence, a loss over the complete image is more appropriate. And, we use the image reconstruction loss $\mathcal{L}_{train}$ that utilizes the complete images.
% the depth corresponding to the complete image. 
% The effectiveness of this choice is substantiated in section \ref{sec:results_mask_trainig_target}. 



% % \subsection{Masked Image Modelling (MIM)}
% % We mask the token embeddings of the depth network using blockwise masking as shown in Figure ~\ref{fig:architecture}. The masked portions are replaced with a mask embedding that is learned. The masked and unmasked patches are together fed into the Transformer blocks.  The network learns to predict depth for the complete image by looking at the global context and learning to predict depth for the masked as well as the unmasked portions using only the umasked portions of the image, urging the network to learn more robust relationships. Particularly, we use mask patch size of $16 \times 16$ corresponding to the patch size of the DeIT backbone. We use a mask ratio of 25\% and a blockwise masking strategy. This strategy prevents the network from focusing on short-range dependencies which would allow inpainting depth from those of nearby pixels. We show later that masking the pose networks is however not helpful, as it already looks at the global context and builds relations across different regions of the images. Masking the input to the pose network reduces the available context and decreases the improvements due to the masked image modeling in the depth network. 


% \begin{algorithm}[tbh]
% \footnotesize
% \DontPrintSemicolon
% \SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
% \SetKwFunction{Random}{random}
% \SetKwFunction{Gaussian}{$\mathcal{N}$}
% \SetKwFunction{repeat}{repeat}

% \SetKwRepeat{Do}{do}{while}

% \SetKwData{h}{h}
% \SetKwData{w}{w}
% \SetKwData{MaskRatio}{mask\_ratio}
% \SetKwData{MaskSize}{mask\_size}
% \SetKwData{NumPatches}{num\_patches}
% \SetKwData{MaskRatio}{mask\_ratio}
% \Input{
% unmasked tokens $x_u$ \\
% \MaskSize \\
% \MaskRatio \\ 
% image shape (\h $\times$ \w)
% } 

% \Output{masked tokens $x_m$}
% \BlankLine

% \NumPatches $\leftarrow$ $\frac{\h \times \w}{\MaskSize^2}$ \\
% M $\leftarrow$ [] \\
% \Do{$|M| <$ \MaskRatio $\times$ \NumPatches}{
% s $\leftarrow$ \Random(\MaskSize, \MaskRatio $\times$ \NumPatches $- |M|$) \tcp{Select Block size} 
% r $\leftarrow$ \Random(0.3, $\frac{1}{0.3}$) \tcp {Select Block aspect ratio}
% a $\leftarrow$ $\sqrt{s \cdot r}$; b $\leftarrow$ $\sqrt{s/r}$\\
% y $\leftarrow$ \Random(0, \h - a); x $\leftarrow$ \Random(0, \w - b)\\
% M $\leftarrow$ M $\sqcup$ \{ $(i,j): i \in [y, y+a], j \in [x, x+b]  $\} \tcp{Add Block to mask}
% }
% $M$ = \repeat($M$, $\h//\MaskSize$, $\w//\MaskSize$) \tcp{Repeat mask to match the transformer patch size}
% $x_m$ $\leftarrow$ $x_u \times (1-M) $ + \Gaussian$(0, 0.02) \times M$ \tcp{Generate masked tokens}
% \KwRet{$x_m$}
% \caption{Blockwise Masking for Depth Estimation Network}
% \label{alg:blockwise_masking_depth}
% \end{algorithm}

% % \subsubsection{Masking strategy}

% % \subsubsection{Mask ratio and size}

% % \subsubsection{MIM for Depth Network}

% % \subsubsection{MIM for Pose Network}

% % \subsection{Loss function}
% % SimMIM shows that in order to learn representations that assist in downstream tasks, it is better to learn to predict over the masked patches rather than the complete image as it would waste learning capability on reconstructing a better image. However, when we use the masked image modelling during training of the depth network, the objective is to learn pixelwise dense prediction. Hence a loss over the complete image is more appropriate. Hence, we use an image reconstruction loss that utilizes the depth corresponding to the complete image. 

==> MIMDepth ICRA 2023/files/related_works.tex <==
\section{Related Works}

% Masked language modelling proposed in BERT substantially improved pre-training for transformer-based language models. It has also been extended to transformers for autoencoding high level semantic relationships.   Particularly, blockwise masking that mitigates wastage of modelling capabilities on  short-range dependencies and high-frequency details has shown promising self-supervised solution for leveraging large-scale image data. Recently, it was shown that even random masking with a higher mask ratio or mask size can similarly assist in enhanced self-supervised pre-training from image data.
% However, the inductive biases introduced by such masked image modeling has not been extended to the training regime for the downstream tasks. 

\textbf{Self-supervised Monocular Depth Estimation}
One of the challenging tasks of interest in 3D scene understanding is monocular depth estimation. Although self-supervised depth estimation was introduced for stereo pairs~\cite{godard2017unsupervised}, it was soon extended to a monocular setup~\cite{zhou2017unsupervised}. 
% The self-supervised monocular depth estimation network is trained simultaneously with the monocular ego-motion estimation network. The outputs of the networks are used to warp neighboring image frames in a video which can be compared with the unwarped original target to minimize the photometric error between them~\cite{wang2004image}.  
Monocular self-supervised approaches to depth estimation have the advantage of not requiring any labels and can learn from a wide variety of data from multiple sources. 
% However, this limits the method to utilize only neighboring image frames which don't have high illumination variance~\cite{bian2021unsupervised}. 
Over the years, improvements have been made to deal with challenges due to occlusions~\cite{godard2019digging}, dynamic objects~\cite{gordon2019depth, klingner2020selfsupervised, ranjan2019competitive}, and scale-consistency issues~\cite{bian2019unsupervised,chawlavarma2021multimodal} and more. While most methods generally used 2D convolutional architectures, a 3D convolutional architecture was proposed to estimate depth from symmetrical packing and unpacking blocks that preserve depth details~\cite{guizilini20203d} . Recently, MTSfMLearner~\cite{visapp22} has shown that transformers can also be used for depth and pose estimation resulting in comparable performance, but improved robustness to natural corruptions and adversarial attacks due to their global receptive fields. Although other methods that use transformers have also been proposed~\cite{guizilini2022multi, yang2022depth}, they do not consider the robustness of their proposed approaches.  We show that integrating mask image modeling trains networks to identify long-range dependencies and could further improve the robustness of depth estimation. 

\textbf{Masked Image Modeling}
Masked image modeling is a method for self-supervised representation learning through images corrupted by masking. This was developed following masked language modeling (MLM)~\cite{kenton2019bert}. These methods are based on replacing a portion of the tokenized input sequence with learnable mask tokens and learning to predict the missing context using only the visible context.  iGPT~\cite{chen2020generative} operates on clustered pixel tokens and predicts unknown pixels directly. ViT~\cite{dosovitskiy2020vit} explores masked patch prediction by predicting the mean color.  On the contrary, BEIT~\cite{bao2021beit} operates on image patches but uses an additional discrete Variational AutoEncoder (dVAE) tokenizer~\cite{ramesh2021zero} to learn to predict discrete tokens corresponding to masked portions.  BEIT uses special blockwise masking that mitigates the wastage of modeling capabilities on short-range dependencies and high-frequency details similar to BERT. Instead, SiMMIM~\cite{xie2022simmim} and MAE~\cite{he2022masked} show that even random masking with a higher mask ratio or mask size can similarly perform well for self-supervised pretraining from image data. 
% MAE~\cite{he2022masked} also uses random masking with high mask ratio and shows that autoencoding the image patches results in good representation learning. 
However, MIM has not been explored for directly training a relevant task of interest rather than as a pre-training method. We demonstrate how it can be adapted to improve the robustness of self-supervised monocular depth estimation. 

% A set of challenging training tasks include monocular depth and ego-motion estimation. First proposed by Zhou et al., the depth and ego-motion estimation networks are trained as auxiliary tasks simultaneously by minimizing the image reconstruction error of adjacent images in videos. These self-supervised monocular methods generally have to deal with occlusions, dynamic objects, and scale-consistency issues. Several methods have proposed varying loss functions, and auto-filtering strategies to deal with these problems. Guizlini et al. proposed a 3D convolutional architecture for estimating depth from symmetrical packing and unpacking blocks that preserve depth details. Recently, it has been shown that transformers can also been used for depth and pose estimation resulting in comparable performance, but an improved robustness. Transformers that use multiple frames for depth estimation along with geometric constrains between the frames have also been proposed. Here, we demonstrate how BERT-inspired masked image modelling can be incorporated into self-supervised depth estimation network to result in further improvements in robustness to natural corruptions and adversarial attacks. 
